Derivation of Closed Form of Expected Improvement for Gaussian Process Trained on Log-Transformed Objective

Expected Improvement (EI) is arguably the most widely used acquisition function in Bayesian optimization. However, it is often challenging to enhance the performance with EI due to its sensitivity to numerical precision. Previously, Hutter et al. (2009) tackled this problem by using Gaussian process trained on the log-transformed objective function and it was reported that this trick improves the predictive accuracy of GP, leading to substantially better performance. Although Hutter et al. (2009) offered the closed form of their EI, its intermediate derivation has not been provided so far. In this paper, we give a friendly derivation of their proposition.

==> sections/abstract/main.tex <==
\begin{abstract}
  Around 150 -- 250 words.
\end{abstract}


==> sections/background/main.tex <==
\section{Background}
\subsection{Preliminaries}


==> sections/conclusions/main.tex <==
\section{Conclusions}

==> sections/experiments/main.tex <==
\section{Experiments}

==> sections/introduction/main.tex <==
\section{Introduction}
Random Search~\cite{bergstra2012random}.

\begin{equation}
\begin{aligned}
  f(x) &= x \\
  g(x) &= x^2
\end{aligned}
\label{main:introduction:eq:demo}
\end{equation}


==> sections/methods/main.tex <==
\section{Methods}


==> sections/misc/acknowledgements.tex <==
\section*{Acknowledgements}


==> sections/misc/check-list.tex <==
\section{Checklist}

==> sections/related-work/main.tex <==
\section{Related work}

